Beatnik: A Novel Global Communication Mini-Application

Beatnik is a novel open source mini-application that exercises the complex communication patterns often found in production codes but rarely found in benchmarks or mini-applications. It simulates 3D Raleigh-Taylor instabilities based on Pandya and Shkoller's Z-Model formulation using the Cabana performance portability framework. This paper presents both the high-level design and important implementation details about Beatnik along with four benchmark setups for evaluating different aspects of HPC communication system performance. Evaluation results demonstrate both Beatnik's scalability on modern accelerator-based systems using weak and strong scaling tests up to 1024 GPUs, along with Beatnik's ability to expose communication challenges in modern systems and solver libraries.

==> tables/table_rmse_multi.tex <==
\begin{table}[]
    \centering
    \caption{Root mean square error (RMSE) of cutoff solver, multi-mode}
    \label{table:rmse-multi}
    \hline
    \begin{tabular}{p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth}}
     Implementation & TS 50 & TS 75 & TS 100 \\
\hline
Cutoff-1.00 & 0.0106 & 0.0232 & 0.0502 \\
Cutoff-0.75 & 0.0125 & 0.0302 & 0.068 \\
Cutoff-0.50 & 0.0116 & 0.0288 & 1.43E+48 \\
\hline




    \end{tabular}
\end{table}


==> tables/table_rmse_single.tex <==
\begin{table}[]
    \centering
    \caption{Root mean square error (RMSE) of cutoff solver, single mode}
    \label{table:rmse-single}
    \hline
    \begin{tabular}{p{0.18\linewidth} p{0.12\linewidth} p{0.12\linewidth} p{0.12\linewidth} p{0.12\linewidth} p{0.12\linewidth}}
    Implementation & TS 50 & TS 75 & TS 100 & TS 150 & TS 200 \\
\hline
Cutoff-1.00 & 0.0019 & 0.0055 & 0.013 & 0.0456 & 0.0925 \\
Cutoff-0.75 & 0.4776 & 0.4826 & 0.4929 & 0.0723 & 4.8E+94 \\
Cutoff-0.50 & 0.4781 & 0.4848 & 1.43E+48 & - & - \\
\hline


    \end{tabular}
\end{table}

